LightChain: Scalable DHT-Based Blockchain

As an append-only distributed database, blockchain is utilized in a vast variety of applications including the cryptocurrency and Internet-of-Things (IoT). The existing blockchain solutions show downsides in communication and storage scalability, as well as decentralization. In this article, we propose LightChain , which is the first blockchain architecture that operates over a Distributed Hash Table (DHT) of participating peers. LightChain is a permissionless blockchain that provides addressable blocks and transactions within the network, which makes them efficiently accessible by all peers. Each block and transaction is replicated within the DHT of peers and is retrieved in an on-demand manner. Hence, peers in LightChain are not required to retrieve or keep the entire ledger. LightChain is fair as all of the participating peers have a uniform chance of being involved in the consensus regardless of their influence such as hashing power or stake. We provide formal mathematical analysis and experimental results (simulations and cloud deployment) to demonstrate the security, efficiency, and fairness of LightChain , and show that LightChain is the only existing blockchain that can provide integrity under the corrupted majority power of peers. As we experimentally demonstrate, compared to the mainstream blockchains such as Bitcoin and Ethereum, LightChain requires around 66 times smaller per node storage, and is around 380 times faster on bootstrapping a new node to the system, and each LightChain node is rewarded equally likely for participating in the protocol.

==> sections/results/analysis.tex <==
\subsection{Security Analysis}
In this section, we analyze the Security, Liveness, and Availability of \textit{\lightchain} system. For the sake of page limit, we skip the intermediate steps of the analysis and refer the interested readers to the full version of this paper \cite{hassanzadeh2019lightchain} where we present the analytical framework with the intermediate steps.

\textbf{Definition 1 ($\adv$-security)} A blockchain system is $\adv$-secure, if for each probabilistic polynomial time adversary \texttt{A} that adaptively controls a fraction $\adv$ of the nodes, the probability that \texttt{A} forks a history or commits an adversarial transaction or block to the blockchain is bound by $\epsilon(\lambda)$, where $\lambda$ is the security parameter of system and $\epsilon$ is a negligible function in $\lambda$. 

\noindent\textbf{Corollary 1 ($\adv$-security)} Given a system with a partial synchronous network, and an authenticated routing mechanism (as defined in Section \ref{lightchain:sec_preliminaries}), where the honest nodes follow the \lightchain protocols as specified and maintain their availability and responsiveness in the system, and considering the negligible function $\epsilon(\lambda)= 2^{-\lambda}$, there exists values of \textit{Validators Threshold} $\validatorThreshold$ and \textit{Signatures Threshold} $\signatureThreshold$, which make the \lightchain $\adv$-secure as shown by Equations \ref{lightchain:eq_alpha} and \ref{lightchain:eq_tm}.

\begin{align}
    \validatorThreshold &\geq \frac{(\sqrt{ \adv} + \sqrt{\adv \times (\psi^{-1}(1- 2^{-\lambda}))^{2} + 4}))^{2}}{4(1-\adv)}
    \label{lightchain:eq_alpha} \\
     \signatureThreshold &\geq (\sqrt{\validatorThreshold \adv(1-\adv)} \times \psi^{-1}(1- 2^{-\lambda})) + \validatorThreshold \adv + 1
     \label{lightchain:eq_tm}
\end{align}

\textbf{Definition 2 ($\adv$-Liveness)} A blockchain system provides $\adv$-liveness, if for each probabilistic polynomial time adversary \texttt{A} that adaptively controls a fraction $\adv$ of the nodes, the probability that \texttt{A} prevents honest nodes from committing their transactions or blocks to the blockchain is bound by $\epsilon(\lambda)$, where $\lambda$ is the security parameter of system and $\epsilon$ is a negligible function in $\lambda$. 

\textbf{Corollary 2 ($\adv$-Liveness)} Given a system with a partial synchronous network, and an authenticated routing mechanism (as defined in Section \ref{lightchain:sec_preliminaries}), where the honest nodes follow the \lightchain protocols as specified and maintain their availability and responsiveness in the system, considering the negligible function $\epsilon(\lambda)= 2^{-\lambda}$, given \textit{Validators Threshold} $\validatorThreshold$, there exists value of \textit{Signatures Threshold} $\signatureThreshold$, which makes the \lightchain provide $\adv$-liveness as shown by Equations \ref{lightchain:eq_efficiency}.

\begin{equation}
    t \leq \frac{\validatorThreshold(1-\adv)(1- \ufp)}{\adv + (1 - f)(1 - \ufp)}
    \label{lightchain:eq_efficiency}
\end{equation}

\textbf{Definition 3 (Availability:)} A blockchain system provides availability, if at least a single copy of each committed transaction and block remains available over the time. 

\textbf{Corollary 3 (Availability)} Given a system with a partial synchronous network, and a uniform and independent failure probability of $\ufp$ for the honest peers of the system, there is a value for the \textit{Signatures Threshold} $\signatureThreshold$ as shown by Equation \ref{lightchain:eq_replica_availability} by which \lightchain provides availability by replicating a validated transaction or block on its owner as well as \signatureThreshold validators.

\begin{equation}
    t \geq \frac{1}{1-q} - 1
    \label{lightchain:eq_replica_availability}
\end{equation}



 

